BERTHA: Video Captioning Evaluation Via Transfer-Learned Human Assessment

Evaluating video captioning systems is a challenging task as there are multiple factors to consider; for instance: the fluency of the caption, multiple actions happening in a single scene, and the human bias of what is considered important. Most metrics try to measure how similar the system generated captions are to a single or a set of human-annotated captions. This paper presents a new method based on a deep learning model to evaluate these systems. The model is based on BERT, which is a language model that has been shown to work well in multiple NLP tasks. The aim is for the model to learn to perform an evaluation similar to that of a human. To do so, we use a dataset that contains human evaluations of system generated captions. The dataset consists of the human judgments of the captions produce by the system participating in various years of the TRECVid video to text task. These annotations will be made publicly available. BERTHA obtain favourable results, outperforming the commonly used metrics in some setups.

==> sec999_extra.tex <==
\subsection{Qualitative analysis}

Apart from the quantitative analysis present previously, a qualitative analysis is also interesting to understand how the model performs. To prepare this analysis, we focus on using the word cloud to see which words are more relevant for each metric. The phrase cloud consists of the top 10 scoring pair of references-system generated caption. Each sentence is divided into words. Without performing any tokenisation, the words are used to compute the cloud. The cloud represents the most mention word as the most prominent word in terms of text size. The only words remove from this plot are the common stop-words that do not add any information, words like "in", "us", or "a". In figure ~\ref{fig:wc0} all the word clouds for the metrics are presented for the year TTV-20 of the MA dataset. It can be observed that metrics base on n-grams share similar behaviour and give importance to similar words.

Analysing the results, the first thing to notice is that all the metrics give some importance to words like "man", "young", or "white". Those are the standard topics where a man or a young person is involved in some activity. Except for BERTHA, all the other automatic metrics give a considerable relevance to "dancing" and "shirt", which is not relevant for the human assessment. BERTHA focus on "holding" and "black". They fail to include "talking" as the main activity that humans consider necessary to differentiate good from wrong captions. 

This analysis helps to spot weaknesses in what is essential for each metric compared to the human assessment. In general, metrics that use only the intersection of words between the references and the system generate sentences perform poorly compared to those looking for tendencies or synonyms, which is to be expected as the task is to describe a topic and not a translation with exact words. BERTHA proves that it focuses on some different patterns than the other metrics and gets a high correlation. This implies that BERTHA is an excellent metric to use a compliment for the other ones.

\begin{figure}
    \centering
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.9\linewidth]{figs/TRECvid_TRECvid20-vttMAredoallyears_mx30_me200_1_scores_wordcloud.png}
      \caption{Human assessment}
      \label{fig:wc1}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.9\linewidth]{figs/TRECvid_TRECvid20-vttMAredoallyears_mx30_me200_1_preds_raw_wordcloud.png}
      \caption{BERTHA}
      \label{fig:swc2}
    \end{subfigure}%
    
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.9\linewidth]{figs/TRECvid_TRECvid20-vttMAredoallyears_mx30_me200_1_bleu_raw_wordcloud.png}
      \caption{Bleu-4}
      \label{fig:wc3}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
      \centering
\includegraphics[width=.9\linewidth]{figs/TRECvid_TRECvid20-vttMAredoallyears_mx30_me200_1_cider_raw_wordcloud.png}
      \caption{CIDEr}
      \label{fig:swc4}
    \end{subfigure}%
    
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.9\linewidth]{figs/TRECvid_TRECvid20-vttMAredoallyears_mx30_me200_1_meteor_raw_wordcloud.png}
      \caption{Meteor}
      \label{fig:wc5}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.9\linewidth]{figs/TRECvid_TRECvid20-vttMAredoallyears_mx30_me200_1_rouge_raw_wordcloud.png}
      \caption{Rouge}
      \label{fig:swc6}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.9\linewidth]{figs/TRECVID_trecvid20-vttMAredoallyears_mx30_me200_1_raw_spice_raw_wordcloud.png}
      \caption{SPICE}
      \label{fig:swc7}
    \end{subfigure}
      \caption{Word cloud for TRECvid 2020 MA for the references level }
  \label{fig:wc0}
\end{figure}

==> tbl-7-results-sigwilliams.tex <==

\begin{tabular}{lrrrrrr}
\toprule
  & BERTHA & BLEU-4 & CIDEr & Meteor & ROUGE & SPICE \\
\midrule
BERTHA & - / - & 0.497 / - & - / - & - / - & 0.308 / - & 0.289 / 0.492 \\
BLEU-4    & - / 0.010 & - / -     & - / -  & - / 0.464     & 0.143 / 0.010 & 0.261 / 0.012 \\
CIDEr     &0.213 / 0.000 & 0.013 / -     & - / -     & 0.034 / 0.078     & 0.004 / 0.000 & 0.079 / 0.003 \\
METEOR    & 0.405 / 0.003 & 0.216 / - & - / - & - / -     & 0.007 / 0.000 & 0.199 / 0.009 \\
ROUGE  & - / 0.127     & - / -  & - / - & - / -  &- / - & 0.489 / 0.145 \\    
SPICE  & - / -  & - / -  & - / - & - / -  &- / - & - / -  \\ 
\bottomrule
\end{tabular}
